Incorporating Discriminator in Sentence Generation: a Gibbs Sampling Method

Generating plausible and fluent sentence with desired properties has long been a challenge. Most of the recent works use recurrent neural networks (RNNs) and their variants to predict following words given previous sequence and target label. In this paper, we propose a novel framework to generate constrained sentences via Gibbs Sampling. The candidate sentences are revised and updated iteratively, with sampled new words replacing old ones. Our experiments show the effectiveness of the proposed method to generate plausible and diverse sentences.

==> TB-sst.tex <==
\label{my-label}
\begin{tabular}{l|l|l|l}
Sentiment                 & Gibbs Sampling                  & Beam Search                     & Sample and Discriminate     \\ \hline
\multirow{3}{*}{negative} & Yes , the movie is too bad .    & It ’s a bad movie .             & It 's a bad movie .         \\ \cline{2-4} 
                          & One of the worst of the year .  & It ’s a bad film .              & An awful film .             \\ \cline{2-4} 
                          & The film is a little too long . & It ’s not very funny .          & It 's not a good movie .    \\ \hline
\multirow{3}{*}{positive} & This is a movie that is funny . & A very funny m
ovie .            & A fascinating documentary . \\ \cline{2-4} 
                          & It ’s a great kind of movie .   & It ’s a very funny movie .      & It 's a good movie .        \\ \cline{2-4} 
                          & One of the year ’s best films . & One of the year ’s best films . & It 's a great film .
                          \caption{generated sentences on SST-2}
\end{tabular}

